AutoML-guided Fusion of Entity and LLM-based Representations for Document Classification

Large semantic knowledge bases are grounded in factual knowledge. However, recent approaches to dense text representations (i.e. embeddings) do not efficiently exploit these resources. Dense and robust representations of documents are essential for effectively solving downstream classification and retrieval tasks. This work demonstrates that injecting embedded information from knowledge bases can augment the performance of contemporary Large Language Model (LLM)-based representations for the task of text classification. Further, by considering automated machine learning (AutoML) with the fused representation space, we demonstrate it is possible to improve classification accuracy even if we use low-dimensional projections of the original representation space obtained via efficient matrix factorization. This result shows that significantly faster classifiers can be achieved with minimal or no loss in predictive performance, as demonstrated using five strong LLM baselines on six diverse real-life datasets. The code is freely available at \url{https://github.com/bkolosk1/bablfusion.git}.

==> table_vert.tex <==
\begin{table}[h!]
    \centering
        \caption{Accuracy of Document Representations Across Datasets. \underline{Underlined} entries indicate the model that outperformed others in the given setting, while \textbf{bolded} entries highlight the best overall model. \hl{mogoce lah to tabelo transponiras, bo ful enga prostora prihranjenega}}
    \begin{tabular}{l l c c}
        \toprule
        \textbf{Dataset} & \textbf{Document} & \textbf{Baseline} & \textbf{BabelFusion} \\
        & \textbf{Representation} & \textbf{accuracy}  & \textbf{accuracy} \\
%9415
        \midrule 
        \multirow{5}{*}{Books}     & Angle & 93.85 & \underline{95.40} \\
                                   & OpenAI-small & 94.00 & \underline{94.15}  \\
                                   & OpenAI-large & 93.95 & \underline{\textbf{96.05}} \\
                                   & mxbai & 94.00 & \underline{95.75} \\
                                   & LLM2Vec-LLaMa3 & 92.45 & \underline{93.65} \\
                                    \midrule
        \multirow{5}{*}{DVD}       & Angle & 94.15 & \underline{94.95} \\
                                   & OpenAI-small & \underline{94.15} & 93.90 \\
                                   & OpenAI-large & 94.15 & \underline{95.15} \\
                                   & mxbai & 94.10 & \underline{\textbf{95.35}} \\
                                   & LLM2Vec-LLaMa3 & \underline{92.05} & 92.00 \\
                                    \midrule
        \multirow{5}{*}{Music}     & Angle & 91.65 & \underline{94.25} \\
                                   & OpenAI-small & \underline{93.75} & 93.70 \\
                                   & OpenAI-large & 93.75 & \textbf{95.25} \\
                                   & mxbai & 91.90 & \underline{94.00 }\\
                                   & LLM2Vec-LLaMa3 & 91.65 & \underline{92.95} \\
                                    \midrule
        \multirow{5}{*}{Hatespeech}& Angle & 79.06 & \underline{81.62} \\
                                   & OpenAI-small & \underline{\textbf{83.72}} & 76.97 \\
                                   & OpenAI-large & \underline{\textbf{83.72}} & 75.11 \\
                                   & mxbai & 79.53 & \underline{81.04} \\
                                   & LLM2Vec-LLaMa3 & 76.74 & \underline{79.18} \\
                                    \midrule
        \multirow{5}{*}{MLDoc}     & Angle & 95.42 & \underline{95.90} \\
                                   & OpenAI-small & 96.37 & \underline{96.87} \\
                                   & OpenAI-large & 96.37 & \textbf{97.15 }\\
                                   & mxbai & 95.72 & \underline{96.30} \\
                                   & LLM2Vec-LLaMa3 & \underline{96.52 }& 96.15 \\
                                    \midrule
        \multirow{5}{*}{EN-GINCO}    & Angle & 53.67 &\underline{\textbf{ 59.19}} \\
                                   & OpenAI-small & \underline{54.77 }& 53.30 \\
                                   & OpenAI-large & 54.77 & \underline{55.14} \\
                                   & mxbai & 55.51 & \underline{57.35} \\
                                   & LLM2Vec-LLaMa3 & \underline{57.72} & 56.98 \\
        \bottomrule
        \multicolumn{2}{c}{Average} & $ {85.31}_{\pm 14.65}$ & ${\textbf{85.83}}_{\pm\textbf{14.77}}$ \\ 
        \bottomrule

    \end{tabular}

    
    \label{tab:vertical_split}
\end{table}

